LiDAR Cluster First and Camera Inference Later: A New Perspective Towards Autonomous Driving

Object detection in state-of-the-art Autonomous Vehicles (AV) framework relies heavily on deep neural networks. Typically, these networks perform object detection uniformly on the entire camera LiDAR frames. However, this uniformity jeopardizes the safety of the AV by giving the same priority to all objects in the scenes regardless of their risk of collision to the AV. In this paper, we present a new end-to-end pipeline for AV that introduces the concept of LiDAR cluster first and camera inference later to detect and classify objects. The benefits of our proposed framework are twofold. First, our pipeline prioritizes detecting objects that pose a higher risk of collision to the AV, giving more time for the AV to react to unsafe conditions. Second, it also provides, on average, faster inference speeds compared to popular deep neural network pipelines. We design our framework using the real-world datasets, the Waymo Open Dataset, solving challenges arising from the limitations of LiDAR sensors and object detection algorithms. We show that our novel object detection pipeline prioritizes the detection of higher risk objects while simultaneously achieving comparable accuracy and a 25% higher average speed compared to camera inference only.

==> 2_system_ver_1.tex <==
\section{System overview}

% \jy{This section has not been updated yet.}


% \jy{We need to list the assumption somewhere: LiDAR depth clustering have low rate of FN, object detection result is invariant to partial frames.}
% \ay{Suggestion: Rename Section 2 to System Overview, this is roughly what it is, giving a big picture of the framework. Then also include crisp statements of the assumptions and maybe claims? Basically this should pre-answer doubts that will come when reading section 3 and also prepare reader for what to check for and focus on in section 3}

% Consider an autonomous vehicle equipped with (i) a LiDAR sensor that offers depth information and (ii) a video camera that shares the same field of view. A perception module inspects the video in order to determine the locations and types of nearby objects, so that a path planning and control module can navigate accordingly. We assume that perception and control run on different resources (in other words, in this paper, we do not consider optimization pertaining to the control module) and focus on optimizing the perception module only. As argued in the introduction, it is often the case that perception consumes the bulk of resources anyway. We henceforth assume that the perception module runs on a GPU (e.g., Nvidia Jetson TX2, Jetson Xavier).

% A commonly used neural network architecture for perception is YOLO~\cite{redmon2018yolov3}. YOLO simultaneously (i) localizes each of multiple objects in the scene, and (ii) identifies the type of each object. YOLO admits inputs (video frames) of different sizes, where smaller sizes are processed faster. Since not all parts of the video frame contain equally important objects, there is incentive to send YOLO smaller portions of the scene to speed-up execution. Furthermore, since there may be multiple such portions, a second problem is to determine their execution schedule. The above incentive leads to the formulation of an attention cueing problem.

% The goal of attention cueing is to decide which regions of (each) input video frame to hand over to the (neural-network-based) perception module and at what priority.  Restricting the size of these regions (and prioritizing them) will improve responsiveness to more important elements of the scene, while, at the same time, lowering total resource demand. 


\begin{figure}[t]
\centering
    \includegraphics[width=\linewidth]{images/pipeline_diagram.pdf}
    \caption{LiDAR Cluster First and Camera Inference Later Pipeline.}
    \label{fig:cue}
\end{figure}

% Google slides for pipeline_diagram.pdf: https://docs.google.com/presentation/d/1vd_91zRML0KyheIiL2MOO7f5QS5BHTmxMHzQaUWJz-w/edit?usp=sharing

%source is here (https://docs.google.com/drawings/d/1_ymWK8Ckf8VDQy9OD4dx6EeRhAqtQS2Hk0BwasJcPi4/edit?usp=sharing)
% \subsection{The LiDAR Cluster First and Camera Inference Later Subsystem}
% Our proposed end-to-end attention framework is shown in Figure~\ref{fig:cue}. 
In our proposed framework, the LiDAR 3D point cloud is first processed using a popular fast depth-clustering algorithm~\cite{bogoslavskyi17pfg}.
Based on the output of this algorithm we distinguish between critical and non-critical information in the corresponding camera image.
This module has three components: pre-processing, depth-clustering, and projection.

The pre-processing block takes raw LiDAR 3D point cloud and limits the data range to the field of view of the front camera.
Then the depth-clustering block uses an efficient depth-clustering algorithm~\cite{bogoslavskyi17pfg} to associate depth (distance) information with regions in the 3D LiDAR points clouds.
\ay{we get 3D bounding boxes, not depth information alone so rewrite:
Then the depth-clustering block uses an efficient depth-clustering and cluster segmentation algorithm~\cite{bogoslavskyi17pfg} to generate 3D bounding boxes for objects.
}
This depth information is used to determine criticality in the later camera module.
\ay{remove the line above and add it later}
The returned 3D regions are then projected onto the 2D camera frame using the \textit{projection} block, and shaped into rectangular boxes we call \textit{2D clusters}.
\ay{Add: Each projection from 3D bounding box to camera frame is a 2D box with an associated depth \textit{i.e.} a distance from the AV.
This depth information is used to determine criticality in the later camera module.}
This will generate a list of depth-labeled 2D clusters each of which potentially enclose a single object in the image.
These 2D clusters \ay{boxes} are sent to the camera module for further processing.

\ay{Can also add somewhere near the end: "We refer to these 2D projection boxes with depth information as \textit{cluster box}."}


% \textit{preprocessing} block. 
% The preprocessing box applies methods as using only the LiDAR return that are in the Field of view of the camera.
% Next, the data from the preprocessing block are passed through a \textit{depth clustering} block. The depth clustering algorithm~\cite{bogoslavskyi17pfg} associates depth (distance) information with regions in the 3D LiDAR points clouds. The 3D regions returned by the depth clustering block are then projected onto the 2D camera frame using a \textit{projection} block, and shaped into rectangular boxes we call \textit{attention boxes}. Let the set $\mathcal{B}$ denote the set of all boxes mapped onto the current video frame using the above process, where box $\mathcal{B}_i \in \mathcal{B}$ is distance $d_i$ from the observer. Let each box be assigned a priority, $p_i$, that is a function of distance, $p_i = f(d_i)$. These boxes are then consolidated by the {\em attention consolidation algorithm\/} into a smaller number of bigger boxes, called {\em cluster boxes\/}. These cluster boxes are scheduled for inspection by the perception module running on the GPU. 

%\begin{table}[!t]
%\centering
%\begin{tabular}{|l|l|}
%\hline
%\textit{\textbf{Parameters}}                        & \textit{\textbf{Symbol}} \\ \hline
%\textit{Set of all boxes mapped onto current frame} &  $\mathcal{B}$                        \\ %\hline
%\textit{A box in the current frame}                 &   $\mathcal{B}_i$                       \\ %\hline
%\textit{Priority of ith box}                       & $p_i$                         \\ \hline
%\textit{Distance of ith box}                          &  $d_i$                        \\ \hline
%\textit{\rt{Add others here}}                            &                          \\ \hline
%\end{tabular}
%\end{table}

% Figure~\ref{fig:projection}-a shows an example of initial attention boxes generated by the LiDAR (after preprocessing, depth clustering, and projection) from processing the point cloud of a simple scene. Figure~\ref{fig:projection}-b shows the corresponding cluster boxes. Since the perception module inspects only the content of cluster boxes, we say that attention was directed (i.e., cued) to only a part of the input scene. This offers possibilities for resource savings. Moreover, since these boxes are scheduled such that some may be processed ahead of others, perception should be done in a manner that respects the relative importance of the corresponding parts of the scene. 

However, there are three problems related with the depth clustering module.
First, the number of generated 2D clusters is much more than the actual objects in the scene.
As shown in Figure~\ref{fig:cluster}, one object can return many clusters.
There are also clusters generated by the side wall.
Processing these 2D clusters as they are will be very inefficient.
Second, the clusters tend to be smaller than the size of the object in the image.
Sometimes they only cover partial object, having too few information for the DNN to detect the object correctly.
Third, just like LiDAR's performance will suffer in an adverse weather condition (e.g. fog, rain, snow etc.), the depth-clustering algorithm can miss some objects in bad weather.


We address the first two problems by using a depth-based merge algorithm to create CAZones from 2D clusters.
CAZones are regions in the image that potentially contain objects which the vehicle should avoid. 
Unlike a 2D cluster which correspond to a single object, a CAZone can represents several objects that are close on camera image.
The algorithm will be introduced in more detail in the next section.
Regarding the third problem, we avoid it by limiting our framework to highway, sunny and clear weather driving scenarios in which the depth-clustering module does not have \jy{or low rate?} false negative detections.



The outputs from the LiDAR module are then sent to the camera module for further processing and object detection.
We use YOLOv3~\cite{redmon2018yolov3}, a commonly used neural network architecture for detecting objects in the camera scene.
Other neural networks can be used as well, such as ResNet~\cite{he2016deep}.
The requirement on the neural network is that it should be able to accept variable input sizes.
Due to the constraints of the embedded GPU, only one input size can be running at one time.
\ay{reword: "Due to the constraints of the embedded GPU, only one kernel type and thus only one input size can be run on the GPU concurrently.
"}
Various techniques are introduced to solve the limitation by using a real-world LiDAR data.
\ay{The line above contributes nothing. Section 3 start already reiterates the problems so the this connecting line is not required.}

% A commonly used neural network architecture for perception is YOLO~\cite{redmon2018yolov3}. YOLO simultaneously (i) localizes each of multiple objects in the scene, and (ii) identifies the type of each object. YOLO admits inputs (video frames) of different sizes, where smaller sizes are processed faster. Since not all parts of the video frame contain equally important objects, there is incentive to send YOLO smaller portions of the scene to speed-up execution. Furthermore, since there may be multiple such portions, a second problem is to determine their execution schedule. The above incentive leads to the formulation of an attention cueing problem.


% The problem, however, is that in practice, as shown in Figure~\ref{fig:projection}-a, the initial preprocessing, depth clustering, and 2D projection stages return too many clusters. These boxes need to be consolidated to produce \ay{CAZone as in Fig. ..} those in Figure~\ref{fig:projection}-b). It turns out that attention consolidation is a non-trivial problem because it significantly impacts both \ay{prioritization is better than schedulability in this context?} schedulability and object recognition accuracy. Solving this problem is the main contribution of our work which we explain further in the next section.





\begin{figure}[htb]
\includegraphics[width=3.5in]{images/2D_cluster_CAZones.png}
\caption{2D clusters and merged CAZones. The green boxes are the 2D cluster and the blue boxes are the merged CAZones.}
\label{fig:cluster}
\end{figure}

%\rt{Update the Figure to change to a Picture with car infront as suggested by Professor Sha}

%\rt{Revised Introduction. Will finish this part next. Jiyang we do not have the distance aware queue any more. But rather we now have canvas, right? We should update the figure 1 below accordingly}

%Our proposed end-to-end framework is shown in Figure~\ref{fig:pipeline}. 
%The input data for the system include lidar data and camera data.
%The lidar point cloud data is sent to the depth clustering module which uses the algorithm proposed in ~\cite{bogoslavskyi17pfg} to associate depth (distance) information with regions with physical objects in the 3D LiDAR points clouds. 
%The 3D regions returned by the depth clustering block are then projected onto the 2D camera frame and shaped into rectangular boxes we call cluster boxes.
%The cluster boxes information are then combined with camera video frames for the perception module which runs on GPU.
%Instead of the entire video frame, the perception module will only focus on the cluster box regions in each frame.
%Each cropped image area corresponding to a cluster box is preprocessed to meet input requirements and then sent to the distance aware queue.
%The queue has a fixed number of sub-queues which stores cluster box within a certain range of distance value.
%Each sub-queue is a priority queue where the key is the distance value of each box.
%Boxes in the queue are batched together according to a set of rules and sent to the GPU for object detection.


% In this framework, the LiDAR data are first sent to a \textit{preprocessing} block. 
% The preprocessing box applies methods such as tunnel TO DO WHAT?? \rt{Simon Please expand this. Add any figures that can explain all the details here}.
% Next, the data from the preprocessing block are passed through a \textit{depth clustering} block. The depth clustering algorithm~\cite{bogoslavskyi17pfg} associates depth (distance) information with regions in the 3D LiDAR points clouds. The 3D regions returned by the depth clustering block are then projected onto the 2D camera frame using a \textit{projection} block, and shaped into rectangular boxes we call \textit{attention boxes}. Let the set $\mathcal{B}$ denote the set of all boxes mapped onto the current video frame using the above process, where box $\mathcal{B}_i \in \mathcal{B}$ is distance $d_i$ from the observer. Let each box be assigned a priority, $p_i$, that is a function of distance, $p_i = f(d_i)$. These boxes are then consolidated by the {\em attention consolidation algorithm\/} into a smaller number of bigger boxes, called {\em cluster boxes\/}. These cluster boxes are scheduled for inspection by the perception module running on the GPU. 


%\begin{figure*}[htb]
%\label{fig:pipeline}
%\includegraphics[width=6in]{images/DMS_block.png}
%\caption{System pipeline. (This is borrowed from the attention cueing paper draft and need to be modified to use.)}
        
%\end{figure*}



%\subsection{Understanding the Processing of LiDAR RAW Data}

%\begin{figure}[htb]
%\label{fig:rawlidarproj}
%\includegraphics[width=3.5in]{images/frame_camera_129.png}
%\caption{Projection of 2D LiDAR Clusters onto Image..\\ Todo remove blue boxes\\~}
        
%\end{figure}

%\jy{I thought Simon's paper will focus more on the lidar part. We need to make sure there are not much overlap between all three papers.}

%In this section, we describe how LiDAR returned frame looks like when projected from 3D to 2D plane on the camera image. 
%Please note that LiDAR returns three-sixty degree view of the surroundings. 
%In this work, we project only the cluster boxes that are in the field of view (FOV) of the camera. 
%An example of projection of one of the frame of the LiDAR data onto the corresponding camera image is shown in Figure~\ref{fig:rawlidarproj}. 





%The goal of the proposed system is to reduce the processing time and improved the safety of the perception system by resizing and batching input data.

%Two approaches are used to achieve this goal:
%\begin{itemize}
%    \item Determine the region of interest for each video frame to pass to the perception module (merging)
%    \item For each region of interest, determine its resolution to be used for perception
%    \item Batch objects of same input size across different frames together to achieve more efficient GPU utilization
%\end{itemize}




==> 2_system_ver_2.tex <==
\section{System Overview}

%\ay{Add reference to the figure in the text below.}

%In our proposed pipeline, the 3D point cloud from the LiDAR sensor is fed to the LiDAR module as shown in Figure~\ref{fig:pipeline}. 
Our proposed pipeline consists of LiDAR module and a camera module as shown in Figure~\ref{fig:pipeline}.
The LiDAR module has three components: Pre-processing, Depth Clustering, and Camera Projection.
The output from the LiDAR Module is then passed to the Camera Module which can distinguish critical and non-critical objects in the corresponding camera image by utilizing its various components: Depth-Based Merging, CAZone Downsizing, Composite Image Processing, Run Time Guarantee, and Inference.
In the Lidar Module, we employ LiDAR based depth clustering algorithm~\cite{bogoslavskyi17pfg} 
for performing fast segmentation on 3D point clouds.
For Camera Module's Inference component, we use YOLOv3~\cite{redmon2018yolov3}, a commonly used deep neural network for camera based object detection. 
Any neural network that can accept variable input sizes can be used in the inference component, such as all Fully Convolutional Networks (FCN) like YOLOv3 and ResNet~\cite{he2016deep}.
One of the limitation of the GPU when running different size CAZs is that it only supports running one kernel type and one input size at a time.
Batching of same input size is possible. However, different size kernels cannot run concurrently especially on the Volta GPU used in this work. Our various pre-processing approaches are designed to be flexible, to adapt to the capabilities of a given GPU.
%To address such limitations, we employ various pre-processing approaches in the camera module.}
%Due to the constraints of the embedded GPU, only one kernel type and thus only one input size can be run on the GPU concurrently.

==> 3_camera_ver_1.tex <==
\section{The Camera Module}

\begin{figure}[htb]
\includegraphics[width=3.5in]{images/2D_cluster_CAZones.png}
\caption{2D clusters and merged CAZones. The green boxes are the 2D cluster and the blue boxes are the merged CAZones.}
\label{fig:cluster}
\end{figure}

By employing the real Waymo Open Dataset together with the Depth Clustering algorithm, we discover many practical challenges with the list 2D clusters produced from the LiDAR Module. First of all, the number of generated 2D clusters is much more than the actual objects in the scene due to the fact that Depth Clustering does not perform classification and thus over-segments the clusters, as can be seen in Figure~\ref{fig:cluster}. As a result, processing the 2D clusters as they are would result in inefficiency and poor performance. Secondly, the 2D clusters tend to be smaller than the size of the object in the scene due to the limitations of the LiDAR sensors. Sometimes the 2D clusters only enclose the objects partially, which could result in inaccurately created CAZones and thus affect the inference performance of the Camera Module later down in the pipeline. Third, due to the fact that the performance of the LiDAR sensor would be reduced in adverse weather conditions such as fog, rain, snow, and etc., the performance of the LiDAR module would also be reduced, resulting in missed objects.

In this work, we address the first two practical challenges by devising a Depth-Based Merging algorithm, which generate CAZones from the 2D clusters. Unlike a 2D cluster, which ideally should correspond to a single object, a CAZone encloses several objects by grouping 2D clusters that are close on camera image. We also introduce various other components in the Camera Module that further address the challenges. The weather challenge is outside the scope of this work, and we limit our evaluation to datasets that are on the highway with sunny and clear weather conditions. In the further work, however, we plan to address the environmental challenges by introducing a series of improvements to the LiDAR Module for increased segmentation robustness and accuracy.

==> draft.tex <==
\section{Composite image}

With the help of LiDAR, we can obtain a list of 2D clusters which points to potential obstacles.
We assume that the LiDAR is able to detect all physical objects in the front of the car within the LiDAR range.
To avoid any collision and guarantee the safety of the vehicle, only the cluster area on the images need to be processed by the YOLO.
With this insight, we propose using LiDAR collision clusters to form composite image which include only collision clusters provided from LiDAR.


\subsection{Pre-processing}

Since collision clusters come with different sizes, it is important to: 1. choose a composite image size $S$; 2. find a fit for all collision clusters such that the number of composite image is minimal.
These are crucial to the YOLO processing time. 

We determine the composite image size based on the $max(width,height)$ of all collision clusters and then round it up to the closest multiple of 32.
This makes sure even the largest cluster can fit inside the image.
To take advantage of batching, all composite images have the same size so they can be batched and run in parallel.

For fitting all collision clusters, we adopt a modified version of the First-Fit Decreasing Height (FFDH) algorithm which is aware of cluster depth.
We define close and far away clusters according to a safety distance (depth) based on the vehicle's speed.
We use UK's highway code to obtain this distance, which encapsulates driver's thinking and stopping distance.
All collision clusters within this safety distance are considered as dangerous and are assigned high priority. 
The depth-aware FFDH will first sort high priority and low priority clusters by height separately to form two sorted lists.
Next, it will fit all clusters from the high priority list first, and then fit the low priority list.
This is not optimal in terms of minimal images count, but it has a higher chance of separating the two class of clusters and forming low priority composite images.

To meet run time requirements, the GPU is profiled for its processing time for different input size and batch size.
The result is shown in Table~\ref{tab:gpu_profile}.
The input composite image size and batch size are checked against this table to make sure not overrun occurs.
When run time requirement cannot be met, the algorithm will check if there are low priority clusters and remove them first from the run queue, while high priority composite images will never be removed.
If the input combination is still exceeding run time requirement after removing low priority composite images according to Table~\ref{tab:gpu_profile}, the size of all remaining images are reduced to the size according to the profiled table to achieve the preset bound.
This guarantees run time upper bound at the sacrifice of detection accuracy.


\subsection{Postprocessing}

After obtaining the detection results from YOLO, the results are mapped back to the original full frame image to indicate the location of the obstacles.



% \section{Problem formulation}

% Target: maximize confidence, with shortest execution time.


% Known: input image resolution, full frame YOLO input size, raw cluster boxes, box depth, YOLO execution time for different sizes and batches

% Additional: $E_si$ average model classification confidence for an input segment of size $s_i$ 

% constraints: execution time no larger than full frame execution, 

% For each frame of input image and a corresponding set of cluster boxes $B$ that contains $n$ boxes of various sizes $\left \{ b_1, b_2, ..., b_n \right \}$ provided by lidar depth clustering, choose a set of input sizes $S$ from legal input sizes $L$ and batch images to sizes in $S$ such that the boxes transforms to $\left \{ b_1^{'}, b_2^{'}, ..., b_m^{'} \right \}$ and the overall confidence for this frame is maximized:

% \begin{equation}
%     %  \alpha(\Delta) \; = \; \min_{0 \leq t < H} |aew(t,t+\Delta)|
%      \max R = \sum \omega_i E_{s_j} 
% \end{equation}

% under the constraint that the execution time of all boxes $B$ is smaller than 80\% of orignal input size $s_o$ execution time:

% \begin{equation}
%     %  \alpha(\Delta) \; = \; \min_{0 \leq t < H} |aew(t,t+\Delta)|
%     \sum_{s \in S} C_{s,k} \leq 0.8 \times C_{s_o, 1}
% \end{equation}



% solution: 
% \begin{itemize}
%     \item obtain the max number of distinct sizes allowed for the given platform
%     \item a merge algorithm that guarantees an execution time upper bound by 
%     \begin{itemize}
%         \item upper bound the number of square cluster boxes in a frame. 
%         \item use full frame for execution 
%         \item provide optimized box size selection and batching
%     \end{itemize}
    
% \end{itemize}


% \subsection{Merge algorithm phase 1}

% \begin{itemize}
%     \item merge boxes that overlap a lot
%     \item merge boxes that are small and not very far apart
%     \item change box sizes to standardized sizes
%     \item distance-based downsizing
%     \item batch boxes so distinct sizes are not over the max number allowed
% \end{itemize}



% \begin{table}[]
% \begin{tabular}{|c|l|}
% \hline
% \multicolumn{1}{|l|}{Symbol} & Meaning                    \\ \hline
% $b_i$  & i-th cluster box           \\ \hline
% $L$  & Set of legal image sizes   \\ \hline
% $S$  & Set of chosen image sizes   \\ \hline
% $N$ & Number of boxes in a frame \\
% \hline
% $N$ & Number of boxes in a frame \\
% \hline
% $w_i$ & Criticality weight for box $b_i$ \\
% \hline
% $C_{s,k}$ & Execution time of a batch of k images of size s \\
% \hline
% $E_s$ & Model classification confidence of size s \\
% \hline
% $T$ & Total execution time for one frame \\
% \hline
% \end{tabular}
% \end{table}

